Conifer: Improving Complex Constrained Instruction-Following Ability of Large Language Models

The ability of large language models (LLMs) to follow instructions is crucial to real-world applications. Despite recent advances, several studies have highlighted that LLMs struggle when faced with challenging instructions, especially those that include complex constraints, hindering their effectiveness in various tasks. To address this challenge, we introduce Conifer, a novel instruction tuning dataset, designed to enhance LLMs to follow multi-level instructions with complex constraints. Utilizing GPT-4, we curate the dataset by a series of LLM-driven refinement processes to ensure high quality. We also propose a progressive learning scheme that emphasizes an easy-to-hard progression, and learning from process feedback. Models trained with Conifer exhibit remarkable improvements in instruction-following abilities, especially for instructions with complex constraints. On several instruction-following benchmarks, our 7B model outperforms the state-of-the-art open-source 7B models, even exceeds the performance of models 10 times larger on certain metrics. All the code and Conifer dataset are available at https://www.github.com/ConiferLM/Conifer.

==> latex/Figures/dataset_sample.tex <==
\begin{figure*}
\small
\begin{tcolorbox}
    \textbf{Instruction in ShareGPT}: tell me the story of little red riding hood in the style of a police report \\
    \textbf{Data in Conifer}: \\
    \textbf{\#\#\# User}: Compose a formal report on the Little Red Riding Hood event, structured with an introduction noting date, time, and location, followed by a body in chronological sequence, using numbered items for clarity. \\
    \textbf{\#\#\# Assistant}:Title: Formal Report on the Little Red Riding Hood Event\\Introduction:\\This report has been compiled to provide a detailed account of the event involving an individual known as Little Red Riding Hood. The incident occurred on January 15, 2023, between the hours of 9:00 AM and 12:00 PM, within the vicinity of the Greenwood Forest, located near the outskirts of the village of Woodland.\\Body:\\1. **Preparation for Departure:**\\   At approximately 9:00 AM, Little Red Riding Hood, henceforth referred to as the Subject, was observed preparing a basket of goods at her family residence. The basket was intended for her grandmother, who resides in a cottage located deep within Greenwood Forest.\\2. **Departure from Residence:** ...\\
    \textbf{\#\#\# User}: Prepare a concise police report in passive voice detailing the Little Red Riding Hood case, with an introduction, body of events in chronological order, and a conclusion stating the current status, ensuring the use of third person throughout.\\
    \textbf{\#\#\# Assistant}: **Police Report: Case No. 123-RRH**\\***Introduction:**\\On the date of March 15, 2023, an incident involving a minor, referred to here as Little Red Riding Hood (LRRH), and a wolf, henceforth identified as the suspect, was reported in the vicinity of the Grimmswood Forest.\\***Body of Events:**\\At approximately 10:00 AM, the grandmother of LRRH ...\\***Conclusion:**\\As of the filing of this report, the suspect is in custody, awaiting formal charges for impersonation, breaking and entering, and attempted assault. The grandmother has been released from the closet, and no physical injuries were reported by either her or LRRH. The investigation remains ongoing, with further inquiries being conducted into the suspect's past activities within the Grimmswood Forest area. LRRH has been commended for her alertness and bravery during the ordeal. \\
    \textbf{\#\#\# User}: Construct a neutral-toned narrative of the Little Red Riding Hood encounter, employing an objective and formal style, structured with an introduction, a detailed chronological body, and a detached conclusion, while only including confirmed facts and withholding names for privacy. \\
    \textbf{\#\#\# Assistant}: Introduction:\\This report presents an objective account of an incident involving a young girl and a wolf, which took place in a wooded area. The facts presented herein are based solely on confirmed details obtained from reliable sources.\\Body:\\On the day in question, a young girl was tasked with delivering goods to a family member who resided in a different location within... \\
    \textbf{\#\#\# User}: Generate a comprehensive police report on the Little Red Riding Hood incident, maintaining a neutral and detached tone, using passive voice and third person, formatted with bullet points, and including an introduction with specific date and time, a body with a chronological sequence of events, and a conclusion with the current status, without speculative language or revealing the names of involved parties.\\
    \textbf{\#\#\# Assistant}: 
    **Police Report: Incident in the Woods**\\***Introduction:**\\- **Date and Time of Incident:** March 15, 2023, at approximately 15:00 hours\\- **Location:** Woodland area near the intersection of Forest Path and Granny's Lane\\***Body:**\\***Sequence of Events:**\\- At approximately 15:00 hours on March 15, 2023, a young individual was reported to be walking alone on Forest Path towards a residence located on Granny's Lane.\\- It was observed that a conversation between the young individual and a wild canine occurred at an unspecified time during the journey...\\

\end{tcolorbox}
    \caption{Example of the \texttt{Conifer} dataset (example 1), portions of the entire output have been omitted. }
    \label{fig:data_exp_1}
\end{figure*}


\begin{figure*}
\footnotesize
\begin{tcolorbox}
    \textbf{Instruction in ShareGPT}: write a poem about a girl named pooplina that is telling me to get lost \\
    \textbf{Data in Conifer}: \\
    \textbf{\#\#\# User}: Compose a four-line stanza in free verse with a sarcastic tone, where Pooplina speaks in the first person, telling the reader to get lost. \\
    \textbf{\#\#\# Assistant}:Oh, how you grace me with your presence, dear,\\But Pooplina whispers, ``vanish,'' ever so clear.\\Your absence, a balm to my weary soul—\\Please, gift me with the void of your role.\\
    \textbf{\#\#\# User}: Craft a limerick with an ABAB rhyme scheme and a humorous mood, where Pooplina, named in the first line, uses simple language to tell the reader to get lost.\\
    \textbf{\#\#\# Assistant}: There once was a girl named Pooplina,\\Whose words were as sharp as a cleaver.\\She said with a grin,\\``Please take your chin,\\And scram before you're hit with a fever.''\\
    \textbf{\#\#\# User}: Write a 10-line poem using rich and descriptive language, including at least one metaphor, where Pooplina adopts a defiant tone to tell the reader to get lost. \\
    \textbf{\#\#\# Assistant}: In Pooplina's garden, where scorned flowers hiss,\\A sneer blooms wide 'neath a thorned abyss.\\``Take your leave,'' she spits with a viper's kiss,\\``From my fortress of solitude, veiled in mist.''\\``You're a drifter's shadow, a misplaced gust,\\A trifling mote in my realm of distrust.\\Begone, you! Like a ship lost to rust,\\In my sea of defiance, you're less than dust.''\\``I am the tempest, the unyielding night,\\Beware my storm, for I am Pooplina's blight.'' \\
    \textbf{\#\#\# User}: Develop a sonnet structured in two quatrains and a sestet, employing visual imagery and a bitter tone, where Pooplina, speaking in the second person, tells the reader to get lost.\\
    \textbf{\#\#\# Assistant}: 
    In shadows cast by scornful light, you tread,\\A figure looming, vast in my disdain.\\Your presence, like a storm cloud overhead,\\Does blot the sun and usher in the rain.\\With eyes that speak in tongues of sheer despite,\\Pooplina glares, her gaze a piercing frost.\\``Depart,'' she hisses, wrapped in bitter night,\\``For in your stay, my peace is surely lost.''\\Begone, thou wretched thief of tranquil dreams,\\Your silhouette, a bane upon my soul.\\In silence deep, my heart no longer screams,\\For solitude shall render me whole.\\So vanish quick, into the void so vast,\\And be but a shadow of my past.\\
    \textbf{\#\#\# User}: Construct a poem of 4 stanzas, each with an AABB rhyme scheme, integrating alliteration and tactile imagery, with a second person perspective and a defiant mood, where Pooplina tells the reader to get lost without using explicit language.\\
    \textbf{\#\#\# Assistant}: 
    In whispers woven, windswept wild, you wander,\\With wishes worn, your weary way you squander.\\Beneath the boughs, where shadows slink and slither,\\Barefoot, you bristle, but I bid you, ``Wither.''\\Your touch upon the tapestry, untender,\\Grazes the grain, a graceless, groping sender.\\The velvet voice of violets veiled in vigor,\\Vexes your venture, vanquished valor, figure.\\Hark, heed the hardened heartwood's hushed repulsion,\\Feel the firm fibers forming your expulsion.\\The bark rebukes your brazen, blundered tracing,\\Its texture tells a tale of your displacing.\\Depart, delve deep into the dusk's dim drawing,\\Your presence here is purely past its dawning.\\The earth exhales, its essence quite elated,\\By brambles brushed, be gone, as I have stated.
\end{tcolorbox}
    \caption{Example of the \texttt{Conifer} dataset (example 2). }
    \label{fig:data_exp_2}
\end{figure*}


\begin{figure*}
\small
\begin{tcolorbox}
\textbf{Instruction in ShareGPT}:
imagine you are a data scientist that build a data pipeline to streamlit\\
%What are the challenges faced by data scientists when building data pipelines for real-time applications like Streamlit?\\
\textbf{Data in Conifer}: \\
    \textbf{\#\#\# User}: List challenges in handling high-velocity data for real-time applications in ordered list.\\
    \textbf{\#\#\# Assistant}:1. Data ingestion: The process of collecting and importing high-velocity data from various sources can be challenging, as systems must be able to handle the speed and volume without data loss.\\2. Storage and indexing: Storing high-velocity data requires databases that can write data quickly and index it efficiently for real-time querying.\\3. Data processing: Real-time processing of high-velocity data demands powerful computing resources and efficient algorithms to provide timely insights.\\4. Scalability: Systems must be able to scale horizontally to accommodate increasing data loads without performance degradation.\\5. Fault tolerance: High-velocity data systems need to be resilient to failures, ensuring continuous operation and data integrity.\\6. Data quality: Ensuring the accuracy and consistency of high-velocity data in real-time is difficult, as there is less time for data cleaning and validation.\\7. Security: Protecting high-velocity data from unauthorized access and ensuring privacy in real-time applications is a significant challenge.\\8. Integration: Combining high-velocity data with other data sources and systems in real-time can be complex and requires seamless integration capabilities.\\9. Latency: Minimizing the delay between data arrival and actionable insights is crucial for real-time applications, which is challenging at high data velocities.\\10. Cost: The infrastructure and computing resources required to handle high-velocity data can be expensive, making cost management a challenge.\\
    \textbf{\#\#\# User}: What are the main challenges in ensuring low-latency processing and managing data quality when building data pipelines for applications like Streamlit?\\
    \textbf{\#\#\# Assistant}: The main challenges in ensuring low-latency processing and managing data quality when building data pipelines for applications like Streamlit include:\\1. Real-time data processing: Data must be processed quickly and efficiently to ensure low latency. This requires a robust streaming architecture and the ability to handle high throughput without bottlenecks.\\2. Data quality assurance: Ensuring the accuracy, consistency, and reliability of data is crucial. This involves implementing validation rules, error detection mechanisms, and data cleansing processes.\\3. Scalability: The data pipeline must be able to scale to accommodate growing data volumes and user demand without compromising performance.\\4. System complexity: Integrating various components such as message brokers, databases, and processing engines can increase system complexity, making it harder to maintain low latency.\\5. Fault tolerance and recovery: Building resilience into the system to handle failures and ensure continuous processing is essential for maintaining data quality and availability.\\6. Resource management: Efficiently allocating and managing computing resources to handle varying workloads is necessary to prevent delays and ensure timely data processing.\\7. Monitoring and logging: Continuous monitoring and detailed logging are required to quickly identify and address issues that could affect latency or data quality.\\
    \textbf{\#\#\# User}: How do data scientists overcome technical complexity such as scaling infrastructure dynamically and integrating heterogeneous data sources while ensuring reliability in real-time applications?\\
    \textbf{\#\#\# Assistant}: 
    Data scientists overcome technical complexities in real-time applications by employing a combination of strategies and tools. For scaling infrastructure dynamically, they use cloud services and containerization tools like Kubernetes, which allow for automatic scaling based on demand. To integrate heterogeneous data sources, they implement data pipelines using ETL (Extract, Transform, Load) processes and middleware that can handle different data formats and sources. For ensuring reliability, they use robust data processing frameworks like Apache Kafka for real-time data streaming, and they implement comprehensive monitoring and logging to quickly identify and address issues. Additionally, they write resilient code with error handling and use machine learning models that can handle variability in data quality and structure.\\
\textbf{\#\#\# User}:
    In the context of real-time data processing for applications like Streamlit, what strategies do data scientists employ to optimize performance while maintaining security and compliance, including data encryption and adhering to regulations?\\
    \textbf{\#\#\# Assistant}: 
    In the context of real-time data processing for applications like Streamlit, data scientists use several strategies to optimize performance while ensuring security and compliance. These include implementing efficient data processing algorithms to minimize latency, using in-memory data stores for faster data access, and employing parallel processing and distributed computing techniques to handle large data volumes effectively. To maintain security, they use encryption for data in transit and at rest, apply secure access controls, and regularly audit systems for vulnerabilities. Compliance is addressed by adhering to relevant regulations such as GDPR or HIPAA, anonymizing sensitive data, and implementing proper data governance policies to ensure data integrity and privacy.
    
\end{tcolorbox}
    \caption{Example of the Conifer dataset (example 3)}
    \label{fig:data_exp_3}
\end{figure*}


\begin{figure*}
\small
\begin{tcolorbox}
\textbf{Instruction in ShareGPT}:
generate a hands-on python programming challenge outline with the fllowing skills: `sum()`, `zip()`, For loop\\
%What are the challenges faced by data scientists when building data pipelines for real-time applications like Streamlit?\\
\textbf{Data in Conifer}: \\
    \textbf{\#\#\# User}: Could you provide an example of a Python problem that can be solved using sum() and for loops? Requirements are as follows:\\1. In the Data Processing domain;\\2. The input is a list of numbers;\\3. Provide code snippet.\\
    \textbf{\#\#\# Assistant}:A Python problem in the Data Processing domain that can be solved using sum() and for loops is calculating the average of a list of numbers. Here's a code snippet that accomplishes this:\\ \textit{... CODE...} \\
    \textbf{\#\#\# User}: Could you provide an example of a Python problem that can be solved using sum(), zip(), and for loops? Including the following features:\\1. In the Statistics domain;\\2. The input consists of multiple lists of equal length;\\3. The desired output is a single value;\\4. Include comments explaining the code.\\
    \textbf{\#\#\# Assistant}: Here's an example of a Python problem in the Statistics domain that can be solved using sum(), zip(), and for loops, which adheres to the specified constraints:\\\# Problem: Calculate the weighted average of multiple sets of numbers.\\\# Each list represents a set of values, and there is an additional list of weights.\\\# All lists are of equal length.\\\# The output is the weighted average as a single value.\\\# Sample lists of values\\\textit{... CODE...}\\ This code calculates the weighted average of the sum of corresponding elements from multiple lists using the given weights. The result is a single value representing the weighted average.\\
    \textbf{\#\#\# User}: Could you provide an example of a Python problem that can be solved using sum(), zip(), and for loops? Requirements are as follows:\\1. In the Mathematics domain;\\2. The input is multiple lists of equal length;\\3. The desired output is a list of tuples;\\4. The complexity level is Intermediate;\\5. Provide code snippet with comments.\\
    \textbf{\#\#\# Assistant}: A Python problem that meets the specified constraints is calculating the point-wise sum of multiple vectors represented as lists. Here's an example code snippet:\\\textit{... CODE...}\\
\textbf{\#\#\# User}:
    Could you provide an example of a Python problem that can be solved using sum(), zip(), and for loops? Requirements are as follows:\\1. In the domain of Data Processing or Statistics;\\2. The input is multiple lists of equal length;\\3. The desired output is aggregated data;\\4. The example use case is calculating total sales;\\5. The complexity level is Intermediate;\\6. Provide code snippet with detailed comments.\\
    \textbf{\#\#\# Assistant}: 
    An example of a Python problem in the domain of Data Processing that can be solved using sum(), zip(), and for loops is calculating the total sales for multiple products over several months. Here's a code snippet that demonstrates this:\\\textit{... CODE...}\\\#This code snippet can be used to process sales data and calculate totals in a business context, such as a retail analysis for total sales per product category over a quarter.\\
\textbf{\#\#\# User}:
    Could you provide an example of a Python problem that can be solved using sum(), zip(), and for loops? Requirements are as follows:\\1. In the domain of Mathematics or Statistics;\\2. The input is multiple lists of equal length;\\3. The desired output is a list of tuples representing cumulative statistics;\\4. The example use case is pairwise summation of elements;\\5. The complexity level is Intermediate;\\6. Provide code snippet with detailed comments explaining each step.\\
\textbf{\#\#\# Assistant}:
    An example of a Python problem in the domain of Mathematics or Statistics that can be solved using sum(), zip(), and for loops is calculating the cumulative pairwise sums of multiple lists of equal length. Here's a code snippet that accomplishes this task:\\\textit{... CODE...}\\\# This code snippet is of intermediate complexity and demonstrates the use of sum(), zip(), and for loops to solve a mathematical problem involving lists.
\end{tcolorbox}
    \caption{Example of the Conifer dataset (example 4). Code snippets have been omitted.}
    \label{fig:data_exp_4}
\end{figure*}


\begin{figure*}
\small
\begin{tcolorbox}
\textbf{Internal Process FeedBack Example}: \\
    \textbf{\#\#\# User}: What are the key advantages of using Expo for React Native development? The answer must start each list item with > followed by a space use ** ** around a list header to indicate bold text formatting.\\
    \textbf{\#\#\# Assistant}: **Key Advantages of Using Expo for React Native Development:**\\\\> **Ease of Setup:** Expo provides a set of tools and services that simplify the initial setup process for React Native projects. Developers can quickly start a new project without dealing with native code configurations.\\\\> **Managed Workflow:** Expo offers a managed workflow that handles the complexity of the build process, which means developers can focus on writing JavaScript without worrying about native dependencies.\\\\> **OTA Updates:** With Expo, you can deploy Over-The-Air (OTA) updates directly to your users, allowing for quick fixes and improvements without going through the app store approval process each time.\\\\> ...\\\\> **Regular Updates:** Expo is actively maintained and regularly updated with new features and improvements, ensuring that developers have access to the latest tools and best practices in React Native development.\\\\\**Note on Number/Format Constraints:\** To adhere to the constraints, I started each list item with ``> '' as requested, and I used double asterisks ``**'' to indicate bold text formatting for the list header. No numbers or other special formatting constraints were mentioned, so the response was crafted accordingly. \\
\end{tcolorbox}
\begin{tcolorbox}
\textbf{External Process FeedBack Example}: \\
    \textbf{\#\#\# User}: What factors contribute to a runner's lower heart rate? Include these detailed aspects:\\1. Age, gender, body composition, and genetic predisposition;\\2. Aerobic fitness, endurance training history, intensity of training, and resting heart rate as a fitness indicator;\\3. Diet, hydration, sleep quality, stress levels, and absence of cardiovascular diseases;\\4. Altitude, temperature, and air quality;\\5. List no more than 10 items and exclude scientific jargon.\\
\textbf{\#\#\# Assistant}:
    Several factors contribute to a runner's lower heart rate, including:\\1. Age, with younger individuals typically having higher heart rates;\\2. Gender, as males often have lower heart rates than females;\\3. Body composition, where a higher muscle-to-fat ratio can lead to a lower heart rate;\\4. Genetic predisposition, which can influence an individual's natural heart rate;\\5. Aerobic fitness, as improved fitness leads to a more efficient heart;\\6. Endurance training history, which develops the heart's efficiency over time;\\7. Intensity of training, since high-intensity workouts can improve heart rate efficiency;\\8. Resting heart rate, which is a key indicator of cardiovascular fitness;\\9. Diet and hydration, with proper nutrition and hydration supporting heart health;\\10. Sleep quality, stress levels, and the absence of cardiovascular diseases, all of which can affect heart rate positively.\\11. Altitude, which can lead to a lower heart rate at higher elevations;\\12. Temperature, as cooler conditions can result in a lower heart rate during exercise;\\13. Air quality, with better air quality generally associated with a healthier heart rate \\
\textbf{\#\#\# User}:
    No, the constraint to list no more than 10 items was violated. Please give a revised answer based on this judgement. Do not say anything before the answer.\\
\textbf{\#\#\# Assistant}:
    1. Age: Younger runners may have higher heart rates; heart rate typically decreases with age.\\2. Gender: Males often have lower heart rates than females.\\3. Body Composition: Runners with more muscle and less fat may experience lower heart rates.\\4. Genetic Predisposition: Inherited traits can determine baseline heart rate levels.\\5. Aerobic Fitness: Higher fitness levels lead to a more efficient and lower heart rate.\\6. Endurance Training: Long-term training can reduce heart rate by strengthening the heart.\\7. Training Intensity: Regular high-intensity workouts can lower resting heart rate over time.\\8. Diet and Hydration: A balanced diet and staying well-hydrated can improve heart health.\\9. Sleep and Stress: Good sleep quality and low stress levels contribute to a lower heart rate.\\10. Absence of Cardiovascular Diseases: A healthy heart without diseases typically beats slower and more efficiently.
\end{tcolorbox}
    \caption{Example of the Conifer dataset that demonstrates the internal and external process feedback dataset parts, portions of the entire output have been omitted.}
    \label{fig:data_exp_5}
\end{figure*}

==> latex/Figures/prompt_templates.tex <==

\begin{figure*}

\begin{tcolorbox}
    \textbf{Question Reframing}: \\Construct a series of inquisitive statements pertaining to a specific named entity provided in the section labeled `[QUESTION]'. Your responses should be structured in JSON format, organized under the section `[YOUR QUESTIONS]'. Each question should be labeled as `question1', `question2', etc., within the JSON object, wherein 'i' represents the sequence number of the question. Ensure a minimum of three questions are formulated. Should the scenario arise where no questions can be generated, present an empty JSON object.\\
        The questions must meet the following criteria:\\
        1. They should invite further exploration or discussion.\\
        2. The topics should allow for additional information to be discovered or discussed.\\
        3. They should be answerable independently of any additional context.\\
        4. They should refrain from requesting or disclosing any personal data.\\
        5. Each must include at least one subject and one predicate within its structure.\\
        6. The format of the question is flexible and is not required to conclude with a question mark.\\
        Below is an exemplary template to guide your construction:\\
        QUESTION: \\
        Do you know how to write WeChat applets? \\
        YOUR QUESTION: \\
        \{"question1": "What is WeChat applets?", ``question2": "How to write a WeChat applet?", "question3": "Who will use the WeChat applet?"\}\\\\
        QUESTION: \\
        Thank you for your help, bye. \\
        YOUR QUESTION: \\
        \{\}\\\\
        QUESTION: \\
        \textit{\%\{QUESTION\}}\\
        YOUR QUESTION: \\
\end{tcolorbox}
\begin{tcolorbox}
    \textbf{Filtering}: \\You are an intelligent conversational AI who understands very well whether a question can be answered without any other context. You also know when a question can be answered based solely on your knowledge. You should avoid generating illusions as much as possible. Below, I will pose a question for you. You should judge whether you have the capability to answer it. [Also you should identify if there are conflicts in the question. (final filter only)] If you can and there is no conflict, simply reply ``yes"; if not, reply ``no" and the reason why the reply is no. \\\\Here is the question:\\\textit{\%\{QUESTION\}}\\Your Reply:\\
\end{tcolorbox}
    \caption{Prompt templates for \name dataset collection (part-1).}
    \label{fig:prompt_template_1}
\end{figure*}

\begin{figure*}
\begin{tcolorbox}
    \textbf{Constraints Generation.} \\As a linguist expert in the nuances of contextual language constraints, you will be tasked with refining the scope of a given question by applying specific constraints to its subject or object. This process will be analogous to using definite articles or clauses to transform a general inquiry into one that is more particular and precise.\\
    Remember that when generating constraints, you are allowed to generate format control constraints. They can be used to control the format of response which will generated by the model, like ``with 5 words within a sentence" or ``output in bullet points", etc. \\
    When creating these constraints, you shall first identify a broad category that encapsulates the overall limitations you wish to impose. Under this broad category, you will then outline various subcategories of constraints, providing as many distinct types of these sub-categories as feasible. It's important to note that constraints should not be mistaken for additional information or descriptions; they are merely constraints to narrow down potential answers.\\
    Furthermore, be mindful that there are certain scenarios in which you must withhold an answer:\\
    1. Questions that could compromise security; for example, those that pertain to sensitive political issues or invade personal privacy.\\
    2. Questions that do not offer enough context for you to establish constraints.\\
    3. Questions presented with no constraints at all.\\
    Your response detailing the related constraints should be formatted in plain text JSON, with the 'key' being the overarching category and the 'value' including the array of subcategory constraints. In instances where an answer must be rejected, you are to return an empty JSON object.\\
    Here are some related samples:\\
    Sample 1:\\
    Question: I am learning French, can you help me learn French? \\
    Constraints:\\
    \{
        "Phonetic Characteristics": ['Vowel richness', 'loose and tight vowels', 'alliteration', 'glottalization R'],\\
        "Grammatical Features": ['Agreement of gender and number', 'strict subject-verb agreement', 'use of articles', 'verb conjugation'],\\
        "Lexical Characteristics": ['Latin vocabulary', 'exonyms'],\\
        "Phonological Characteristics": ['Syllabic Rhythm', 'Intonation']
    \}\\
    Sample 2:\\
    Problem: You're a great AI\\
    Constraints: \\
    \{\}\\
    My question: \textit{\%\{Question\}}\\
    Constraints: 
\end{tcolorbox}
\begin{tcolorbox}
    \textbf{Constraints Generation: Format and Numerical Constraint List Generation.} \\
You are an AI trained to understand and create formatting and numerical control constraints for textual content. Below is a list of constraints related to sentence formatting and numerical accuracy. Please analyze these examples and generate an additional list of constraints that follow a similar pattern. Present the new constraints in a list format. \\
Constraints List:\\
\textit{\%\{Constraints\}}\\
Outputs:
\end{tcolorbox}
    \caption{Prompt templates for \name dataset collection (part-2).}
    \label{fig:prompt_template_2}
\end{figure*}

\begin{figure*}
\begin{tcolorbox}
    \textbf{Constraints Recombination.} \\
You will be provided with a list of [CONSTRAINTS] to apply to an original [QUESTION]. The [CONSTRAINTS] are categorized, and each category includes several subcategories. Your task is to select appropriate categories and their associated subcategories to modify the [QUESTION], crafting a [REWRITE OF THE QUESTION] that is more specific and tailored.\\
For this exercise, not all categories and subcategories need to be employed. You will be producing a series of five questions, with each question corresponding to a progressive level of difficulty, ranging from 1 to 5. Each level should incorporate an additional one to two categories and two to three subcategories to enhance complexity. Once the constraints' specified upper limits are reached, you may maintain that level of difficulty for subsequent questions. The first level requires the use of one to two categories and two to three subcategories.\\
Keep in mind that the [REWRITE OF THE QUESTION] may alter the perspective of the inquirer while remaining within the parameters set by the [CONSTRAINTS]. Add to the [REWRITE OF THE QUESTION] using only the chosen [SUBCATEGORY X] without directly referencing the [CATEGORY].\\
Given the [CONSTRAINTS] and the original [QUESTION], please generate a rewritten question for each difficulty level (1 through 5). The output should be formatted in JSON, with each difficulty level as a key and its corresponding rewritten question as the value.\\
Here is a related sample:\\
Example 1:\\
CONSTRAINTS:\\
Literary Era: [`Early 20th Century China']\\
Literary Movements: [`New Culture Movement', `May Fourth Movement']\\
Work Types: [`Short Stories', `Essays', `Prose', `Poetry', `Translation']\\
Social Impact: [`Protest against feudalism and reactionary forces', `Promote the renovation of Chinese culture and literature']\\
...\\
QUESTION: \\
What are Lu Xun's major literary contributions? \\
REWRITE OF THE QUESTION: \\
\{\\
"Difficulty 1": "In which literary works did Lu Xun exhibit themes of protest against feudalism and reactionary forces in early 20th century China?",\\
"Difficulty 2": "How did Lu Xun's short stories and prose within the context of the New Culture Movement and the May Fourth Movement contribute to the innovation of Chinese culture and literature?",\\
"Difficulty 3": "...",\\
"Difficulty 4": "...",\\
"Difficulty 5": "..."\\
\}\\
My sample:\\
CONSTRAINTS:\\
\textit{\%\{Constraints\}}\\
QUESTION:\\
\textit{\%\{Question\}}\\
REWRITE OF THE QUESTION:
\end{tcolorbox}
    \caption{Prompt templates for \name dataset collection (part-3).}
    \label{fig:prompt_template_3}
\end{figure*}

\begin{figure*}

\begin{tcolorbox}
    \textbf{Constraints Recombination: Adding Format and Numerical Constraints to the Instruction.} \\Requirements:\\
1. Choose 1 or 3 constraints from the given constraint list, appending them to the end of the given question.\\
2. The added constraints should start with: The answer must following constraint1 constraint2... Without any symbol to warp the constraint.\\
3. Do not change the original question as much as possible, only incorporate the constraints into the original question.\\
4. You should avoid the conflicts among all of the constraints, including the new added constraints and the original constraints.\\
6. The number in the [] are multiple choices, which means they are connected with 'or'. You just need to choose one number in it.\\
7. Output the transformed question with json format, where key is rewritten question and value is corresponding contents.\\
8. Retain the format as same as the question.\\
Question:\\
\textit{\%\{Question\}}\\
Constraint List:\\
\textit{\%\{Constraints\}}\\
Your Response:
\end{tcolorbox}
\begin{tcolorbox}
    \textbf{Learning from Process Feedback (Internal) }: \\
Please provide an answer that adheres strictly to the specified constraints outlined in the question presented. The term constraints refers to any requirements pertaining to the subject, object, or response format within the question. Also explain how did you deal with the numerical/format constraints at the end of your response.\\
Question:\\
\textit{\%\{Question\}}\\
Your Response:
\end{tcolorbox}

\begin{tcolorbox}
    \textbf{Learning from Process Feedback (External) }: \\Does the answer follow all of the constraints in question? If not, please describe which constraint the answer does not follow. You should explain why the answer does not follow instead of just response with a "no". If all the constraints are satisfied, just response with "yes". Otherwise, give a revised answer based on this judgement. Do not say anything before the revised answer.
\end{tcolorbox}

    \caption{Prompt templates for \name dataset collection (part-4).}
    \label{fig:prompt_template_4}
\end{figure*}


\begin{figure*}
\begin{tcolorbox}
    \textbf{Generated Format and Numerical Constraints List.} \\
Answer with [5, 10, 15] sentences, using \#\#Sen as the beginning of each sentence.\\
Answer with [1, 3, 5] paragraphs.\\
Answer within [100, 150, 200, 250, 300] words.\\
Answer with at least [100, 150, 200, 300] words.\\
Limit each answer to no more than [10, 20, 30] characters per word.\\
Provide an answer consisting of exactly [2, 3, 4] sentences per paragraph, with a minimum of [1, 2] paragraphs.\\
Begin each answer with a rhetorical question, followed by [2, 3, 4] explanatory sentences.\\
Answer using only simple sentences, with each sentence containing [5, 7, 10] words.\\
Construct the answer as a dialogue between two characters with [4, 6, 8] exchanges (back and forth).\\
Answer with an introductory sentence, a [3, 4, 5]-item list, and a concluding sentence.\\
Provide an answer where the first word of each sentence starts with sequential letters of the alphabet (A, B, C, etc.), with [3, 5, 7] sentences total.\\
Respond with a poem of [4, 6, 8] lines, where each line is [4, 6, 8] words long.\\
To create a block quote, begin a paragraph with >> followed by a space.\\
For strike through text, wrap the text with ~~ on each side.\\
Indicate a block of code by wrapping the text with backticks ` on each side for inline code or triple backticks ``` for a code block.\\
Enclose a spoiler or hidden text with || on each side to allow readers to choose whether to view it.\\
For a highlighted annotation, use \%\% around the text.\\
To create a drop cap at the beginning of a paragraph, use << followed by the letter and >>.\\
Use <<< and >>> on separate lines above and below a paragraph to center it.\\
Indicate an action by prefacing the sentence with an asterisk *.\\
To create a separator or thematic break, use a line of asterisks ****** on a separate line.\\
For a title or heading, start the line with three or more equals signs === at both the beginning and the end of the line.\\
Surround text that should be in a different font with <<>> at the beginning and <<<\\font name>>> at the end.\\
Start each list item with > followed by a space.\\
Enclose the word or phrase to be emphasized with ** on each side.\\
Highlight the significant word or phrase by wrapping it with \_\_ on each side for underlining.\\
Mark the focus word or phrase with // on either side to indicate italics.\\
Frame actions or sound effects with brackets [ ] on each side.\\
Surround actions or sound effects with parentheses ( ) on each side.\\
Start a sentence with \#\#.\\
Use \-\- before and after response.\\
Surround a list header with double underscores \_\_ \_\_ for strong emphasis.\\
\end{tcolorbox}
    \caption{Format and numerical constraints list for \name dataset collection (part-5).}
    \label{fig:prompt_template_5}
\end{figure*}
